Offline Policy Evaluation and Optimization under Confounding

Evaluating and optimizing policies in the presence of unobserved confounders is a problem of growing interest in offline reinforcement learning. Using conventional methods for offline RL in the presence of confounding can not only lead to poor decisions and poor policies, but also have disastrous effects in critical applications such as healthcare and education. We map out the landscape of offline policy evaluation for confounded MDPs, distinguishing assumptions on confounding based on whether they are memoryless and on their effect on the data-collection policies. We characterize settings where consistent value estimates are provably not achievable, and provide algorithms with guarantees to instead estimate lower bounds on the value. When consistent estimates are achievable, we provide algorithms for value estimation with sample complexity guarantees. We also present new algorithms for offline policy improvement and prove local convergence guarantees. Finally, we experimentally evaluate our algorithms on both a gridworld environment and a simulated healthcare setting of managing sepsis patients. In gridworld, our model-based method provides tighter lower bounds than existing methods, while in the sepsis simulator, our methods significantly outperform confounder-oblivious benchmarks.

==> manuscript_files/kz_example.tex <==

\section{History Dependent Confounder Lower Bound}

\textbf{Environments:} Consider 2 MDPs, $\M_1$ and $\M_2$ with $\mathcal{S} = \{s_1,s_2\}$, $\mathcal{A} = \{1, 2\}$ and $\mathcal{U} = \{*\} \cup \left(\cup_{i=1}^H \{1, 2\}^i\right)$.

\textbf{Rewards:} Define rewards to be $r(s_1) = 1, r(s_2) = 0$ in both MDPs.

\textbf{Confounder transitions:}
Remember that we are working with history-dependent confounders. Confounder transitions are deterministic. $u_1 = *$, $u_2 = a_1$, and $u_{h+1} = (u_h, a_{h+1})$ with probability $1$.

\textbf{State transitions:} 
\begin{itemize}
    \item In $\M_1$, we have $\prob(s_2|s,a,u) = 1$ if $u$ is an alternating sequence and $0$ otherwise.
    \item In $\M_2$, $\prob(s_2|s,a,u) = 1$ for all $a,s,u$ and $0$ otherwise.
\end{itemize}

\textbf{Behavior policies:}
The behavior policy in both MDPs is deterministic, depending on the confounder. $\pi_b$ on the first timestep takes $1$ with probability $1/2$ and $2$ with probability $1/2$. If $u = (a_1, a_2, \cdots a_h)$, then $\pi_b(a \mid s, u) = 1$ for $\{a\} = \{1,2\} \setminus \{a_h\}$ and $0$ otherwise. That is, it takes the opposite action of the last action encoding the current confounder.


\textbf{Observed Transitions:}
We therefore observe only the sequences of actions $(1,2,...1,2)$ and $(2,1,...,2,1)$, each with probability $1/2$. The observed behavior policy is $\pi_{b,h}(a \mid s) = 1/2$ at each timestep, 
for any $s,a$. In both MDPs, the behavior policy remains in state $s_2$ all the time and receives a total reward of $0$.


\textbf{Evaluation Policy:}
Let $\pi_e(a \mid s) = 1/2$ for all $s,a$. In $\M_1$, the total reward is $H-1$ with probability $1-2/2^H$ (all non-alternating trajectories) and $0$ with probability $2/2^H$ (all alternating trajectories). In $\M_2$, it is always $0$. So $V_1(\pi_e ; \M_1) = (1-2/2^H)(H-1) = O(H)$, and  $V_1(\pi_e ; \M_2) = 0$.


\textbf{Remark:}
$\Gamma$ is unbounded in this case. 

